Bayesian Optimization of Expensive Nested Grey-Box Functions

We consider the problem of optimizing a grey-box objective function, i.e., nested function composed of both black-box and white-box functions. A general formulation for such grey-box problems is given, which covers the existing grey-box optimization formulations as special cases. We then design an optimism-driven algorithm to solve it. Under certain regularity assumptions, our algorithm achieves similar regret bound as that for the standard black-box Bayesian optimization algorithm, up to a constant multiplicative term depending on the Lipschitz constants of the functions considered. We further extend our method to the constrained case and discuss special cases. For the commonly used kernel functions, the regret bounds allow us to derive a convergence rate to the optimal solution. Experimental results show that our grey-box optimization method empirically improves the speed of finding the global optimal solution significantly, as compared to the standard black-box optimization algorithm.

==> figs/log_WO_constrained_regret.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{purple}{RGB}{128,0,128}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Step},
xmin=0, xmax=20,
xtick style={color=black},
xtick={0,5,10,15,20},
xticklabels={
  \(\displaystyle {0}\),
  \(\displaystyle {5}\),
  \(\displaystyle {10}\),
  \(\displaystyle {15}\),
  \(\displaystyle {20}\)
},
y grid style={darkgray176},
ylabel={\(\displaystyle \log_{10}\)(Constrained Regret) 
(Averaged over 30 instances)},
ymin=-2.27444606995579, ymax=2.32942847449926,
ytick style={color=black},
ytick={-3,-2,-1,0,1,2,3},
yticklabels={
  \(\displaystyle {\ensuremath{-}3}\),
  \(\displaystyle {\ensuremath{-}2}\),
  \(\displaystyle {\ensuremath{-}1}\),
  \(\displaystyle {0}\),
  \(\displaystyle {1}\),
  \(\displaystyle {2}\),
  \(\displaystyle {3}\)
}
]
\path [draw=red, fill=red, opacity=0.3]
(axis cs:0,2.1201614497513)
--(axis cs:0,1.97604168564204)
--(axis cs:1,1.57218866025504)
--(axis cs:2,0.0970311014436785)
--(axis cs:3,-0.681886423986071)
--(axis cs:4,-0.843097252891914)
--(axis cs:5,-1.10683840101713)
--(axis cs:6,-1.37657544070013)
--(axis cs:7,-1.69588664564609)
--(axis cs:8,-1.75821206741376)
--(axis cs:9,-1.84928791181124)
--(axis cs:10,-1.89231057593465)
--(axis cs:11,-1.9794337340681)
--(axis cs:12,-1.99498656437678)
--(axis cs:13,-2.02926049601668)
--(axis cs:14,-2.03927677304412)
--(axis cs:15,-2.05212605292257)
--(axis cs:16,-2.05644989299224)
--(axis cs:17,-2.0595344651677)
--(axis cs:18,-2.06253969806255)
--(axis cs:19,-2.06517904520784)
--(axis cs:19,-1.94445231911896)
--(axis cs:19,-1.94445231911896)
--(axis cs:18,-1.94068862185629)
--(axis cs:17,-1.93643699335076)
--(axis cs:16,-1.93195141262537)
--(axis cs:15,-1.92586773523706)
--(axis cs:14,-1.90646856207752)
--(axis cs:13,-1.89118502103735)
--(axis cs:12,-1.84086514986128)
--(axis cs:11,-1.81743504081998)
--(axis cs:10,-1.76048403593397)
--(axis cs:9,-1.66388886351164)
--(axis cs:8,-1.571583101587)
--(axis cs:7,-1.36654164120341)
--(axis cs:6,-0.675353761870144)
--(axis cs:5,-0.356499029032351)
--(axis cs:4,-0.0470897968930822)
--(axis cs:3,0.137710112442635)
--(axis cs:2,0.839623519554146)
--(axis cs:1,1.78122642930182)
--(axis cs:0,2.1201614497513)
--cycle;

\path [draw=purple, fill=purple, opacity=0.3]
(axis cs:0,1.09174817402723)
--(axis cs:0,0.261532502032416)
--(axis cs:1,0.11179240245253)
--(axis cs:2,-0.225591113405812)
--(axis cs:3,-0.516560913832337)
--(axis cs:4,-0.644915318561814)
--(axis cs:5,-0.717424379124294)
--(axis cs:6,-0.830757971480879)
--(axis cs:7,-0.840548475943402)
--(axis cs:8,-0.863262870747849)
--(axis cs:9,-0.895129343585576)
--(axis cs:10,-0.915420929509673)
--(axis cs:11,-0.926557919942662)
--(axis cs:12,-0.953216637970812)
--(axis cs:13,-0.983368980253668)
--(axis cs:14,-1.01601882567307)
--(axis cs:15,-1.02844544039727)
--(axis cs:16,-1.05648075292194)
--(axis cs:17,-1.07822654477511)
--(axis cs:18,-1.10549840587734)
--(axis cs:19,-1.13394184598647)
--(axis cs:19,-0.477437602765131)
--(axis cs:19,-0.477437602765131)
--(axis cs:18,-0.416358588822337)
--(axis cs:17,-0.362110714894287)
--(axis cs:16,-0.319170020999896)
--(axis cs:15,-0.256194231591856)
--(axis cs:14,-0.232740213851466)
--(axis cs:13,-0.194794982223968)
--(axis cs:12,-0.148390313788194)
--(axis cs:11,-0.095882506832709)
--(axis cs:10,-0.0722066837542213)
--(axis cs:9,-0.0309215083840888)
--(axis cs:8,0.00646734418498734)
--(axis cs:7,0.0410881107982903)
--(axis cs:6,0.0563098004000164)
--(axis cs:5,0.163092381997301)
--(axis cs:4,0.264750809459418)
--(axis cs:3,0.402071435377017)
--(axis cs:2,0.659260631250214)
--(axis cs:1,0.942705286279052)
--(axis cs:0,1.09174817402723)
--cycle;

\addplot [red, mark=o, mark size=0.15, mark options={solid,fill=none}]
table {%
0 2.04810166358948
1 1.67670750617981
2 0.468327283859253
3 -0.272088170051575
4 -0.445093512535095
5 -0.731668710708618
6 -1.02596461772919
7 -1.53121411800385
8 -1.6648975610733
9 -1.7565883398056
10 -1.82639729976654
11 -1.89843440055847
12 -1.91792583465576
13 -1.96022272109985
14 -1.97287261486053
15 -1.98899686336517
16 -1.99420070648193
17 -1.99798572063446
18 -2.00161409378052
19 -2.00481557846069
};
\addlegendentry{Ours}
\addplot [purple, mark=square, mark size=0.15, mark options={solid,fill=none}]
table {%
0 0.676640272140503
1 0.527248859405518
2 0.216834783554077
3 -0.0572447776794434
4 -0.190082311630249
5 -0.27716600894928
6 -0.387224078178406
7 -0.399730205535889
8 -0.42839777469635
9 -0.463025450706482
10 -0.493813753128052
11 -0.511220216751099
12 -0.550803422927856
13 -0.589082002639771
14 -0.624379515647888
15 -0.642319917678833
16 -0.687825441360474
17 -0.720168590545654
18 -0.760928511619568
19 -0.805689811706543
};
\addlegendentry{CONFIG}
\end{axis}

\end{tikzpicture}

